Data augmentation enhanced speaker enrollment for text-dependent speaker verification

Data augmentation is commonly used for generating additional data from the available training data to achieve a robust estimation of the parameters of complex models like the one for speaker verification (SV), especially for under-resourced applications. SV involves training speaker-independent (SI) models and speaker-dependent models where speakers are represented by models derived from an SI model using the training data for the particular speaker during the enrollment phase. While data augmentation for training SI models is well studied, data augmentation for speaker enrollment is rarely explored. In this paper, we propose the use of data augmentation methods for generating extra data to empower speaker enrollment. Each data augmentation method generates a new data set. Two strategies of using the data sets are explored: the first one is to training separate systems and fuses them at the score level and the other is to conduct multi-conditional training. Furthermore, we study the effect of data augmentation under noisy conditions. Experiments are performed on RedDots challenge 2016 database, and the results validate the effectiveness of the proposed methods.

==> References <==
@inproceedings{michelsanti2017conditional,
  title={{C}onditional Generative Adversarial Networks for Speech Enhancement and Noise-Robust Speaker Verification},
  author={Michelsanti, D. and Tan, Z.-H.},
  booktitle={Proc. of Interspeech},
  pages={2008--2012},
  year={2017},
}

@Article{Mahalanobis36,
	author={P. C. Mahalanobis},
	title={{O}n the {G}eneralised {D}istance in {S}tatistics},
	journal={Proc. of the National Institute of Sciences of India},
        volume={2},
	pages={49-55},
	year={1936}
}


@Article{MacQueen67,
	author={J. MacQueen},
	title={{S}ome {M}ethods for {C}lassification and {A}nalysis of {M}ultivariate {O}bservations},
	journal={Proc. Fifth Berkeley Symp. on Math. Statist. and Prob. (Univ. of Calif. Press)},
	volume={1},
	pages={281-297},
	year={1967}
}

@Article{ross74,
	author={M. J. Ross and  H. L. Shaffer and A. Cohen and R. Freudberg and H. J.Manley},
	title={{A}verage {M}agnitude {D}ifference {F}unction {P}itch {E}xtractor},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={22},
	pages={353-362},
	year={1974}
}

@INPROCEEDINGS{Makhoul75,
	author = {J. Makhoul},
	title = {{L}inear {P}rediction: {A} {T}utorial {R}eview},
	booktitle = {Proceedings of the IEEE},
	volume={63},
	pages={561-580},
	year={1975}
}

@Article{Sambur76,
	author = {M. R. Sambur},
	title = {{S}peaker {R}ecognition using {O}rthogonal {L}inear {P}rediction},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={24},
	pages={283-289},
	year={1976}
}
	
@Article{Markel77,
	author = {J. D. Markel and B. T. Oshika and Jr. A. M. Gray},
	title = {{L}ong-term {F}eature {A}veraging for {S}peaker {R}ecognition},
        journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={25},
	pages={330-337},
	year={1977}
}

@Article{dempster77,
  author={A. Dempster and N. Laird and D. Rubin},
  title={{M}aximum {L}ikelihood from {I}ncomplete {D}ata via {EM} {A}lgorithm},
  journal={J. Roy. statist. Soc.},
  volume={39},
  pages={1-38},
  year={1977}
   }

@Article{Davis80,
	author={S. B. Davis and P. Mermelstein},
	title={{C}omparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={28},
	pages={357-366},
	year={1980}
}

@Article{LINDE80,
	author={Y. Linde and A. Buzo and  R. M. GRAY},
        title={{A}n {A}lgorithm for {V}ector {Q}uantizer {D}esign},
	journal={IEEE Trans. Communications},
	volume={28},
	pages={84-94},
	year={1980}
}

@Article{Furui81,
	author={S. Furui},
	title={{C}epstral {A}nalysis {T}echnique for {A}utomatic {S}peaker {V}erification},
	journal={IEEE Trans. on  Acoust. Speech Signal Processing},
	volume={29},
	pages={254-272},
	year={1981}
}

@Article{Rabiner89,
	author={L. R. Rabiner},
	title={{A} {T}utorial on {H}idden {M}arkov {M}odels and {S}elected {A}pplications in {S}peech {R}ecognition},
	journal={Proc. of the IEEE},
	volume={77},
	pages={257-285},
	year={1989}
}



@Article{Hermansky90,
	author={H. Hermansky},
	 title={{P}erceptual Linear Predictive (PLP) Analysis of Speech},
	 journal={J. Acoust. Soc. Am.},
	 volume={87},
	 pages={1738-1752},
	 year={1990}
}

@Article{Higgin91,
author="A. Higgins and L. Bahler and J. Porter",
title="{S}peaker {V}erification using {R}andomized {P}hrase {P}rompting",
journal="Digital Signal Processing",
volume="1",
 pages="89-106",
year="1991"	 
}

@INPROCEEDINGS{reynolds91,
	author = {D. A. Reynolds and L. P. Heck},
	title = {{I}ntegration of {S}peaker and {S}peech {R}ecognition {S}ystems},
         booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {869-872},
	year = {1991}
}


@INPROCEEDINGS{Rosenberg92,
	author = {A. E. Rosenberg and J. DeLong and C\-H Lee and B\-H Jaung and F. K. Soong},
	title = {{T}he {U}se of {C}ohort {N}ormalized {S}cores for {S}peaker {V}erification},
	booktitle = { Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {599-602},
	year = {1992}
}

@Article{Hermanksy94,
       author = {H. Hermanksy and N. Morgan},
       title = {{R}ASTA Processing of Speech},
       journal={IEEE Trans. on Speech and Audio Processing},
       volume={2},
       pages={578-589},
       year={1994}
}

@Article{Gauvain94,
	author = {J.-L. Gauvain and C.-H. Lee},
	title = {{M}aximum a {P}osteriori {E}stimation for {M}ultivariate {G}aussian {M}ixture {O}bservations of {M}arkov {C}hains},
	journal={IEEE Trans. on Speech and Audio Processing},
	volume={2},
	pages={291-298},
	 year={1994}
}


@Article{reynold95,
  author="D. A. Reynolds",
  title="{S}peaker {I}dentification and {V}erification using {G}aussian {M}ixture {S}peaker {M}odels",
  journal="Speech Communication",
  volume="17",
  pages="91-108",
  year="1995"
}

@Article{Leggeter95,
author="C. Leggetter and P. Woodland",
title="{M}aximum {L}ikelihood {L}inear {R}egression for {S}peaker {A}daptation of {H}MMs",
journal="Computer Speech and Language",
volume="9",
pages="171-186",
year="1995"	
}
@Article{Vapnik95,
	author={C. Cortes and V. Vapnik},
	title={{S}upport {V}ector {N}etworks},
	journal={Machine Learning},
	volume={20},
	pages={273-297},
	year={1995}
}

@INPROCEEDINGS{Talkin95,
	author = {D. Talkin},
        title = {{A} {R}obust {A}lgorithm for {P}itch {T}racking ({RAPT})},
	booktitle = {in Speech coding and synthesis (Elsevier, ed.)},
	pages = {495-518},
        year = {1995}
}

@INPROCEEDINGS{leerose96,
 author = {Li Lee and Richard C. Rose},
 title = {{S}peaker {N}ormalization using {E}fficient {E}requency {W}arping {P}rocedures},
 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {353-356},
 year = {1996}
}



@INPROCEEDINGS{Rosenberg96,
	 author = {A. E. Rosenberg and S. Parthasarathy},
	 title = {{S}peaker {b}ackground {m}odels for {c}onnected {d}igit {p}assword {s}peaker {V}erification},
	 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {81-84},
	 year = {1996}
}




@INPROCEEDINGS{LHeck97,
	  author = {L. Heck and M. Weintraub},
	  title = {{H}andset-dependent {B}ackground {M}odels for {R}obust {T}ext-{I}ndependent {S}peaker {R}ecognition},
          booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	  pages = {1071-1074},
	  year = {1997}
}


@INPROCEEDINGS{DET97,
	   author = {A. Martin and G. Doddington and T. Kamm and M. Ordowskiand and M. Przybocki},
	   title = {{T}he DET Curve in Assessment of Detection Task Performance},
	   booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	   pages = {1895-1898},
	   year = {1997}
}  


@INPROCEEDINGS{Ariyaeeinia97,
	author= {A. M. Ariyaeeinia and P. Sivakumaran},
	title = {{A}nalysis and {C}omparison of {S}core {N}ormalization {M}ethods for {T}ext {D}ependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {1379-1382},
	year = {1997}
}


@article{Lee-Rose98,
      author="L. Lee and R. Rose",
      title="{F}requency {W}arping {A}pproach  to {S}peaker {N}ormalization",
      journal="IEEE Trans. on Speech and Audio Processing",
      volume={6},
      pages={49-59},
      year={1998}
}



@INPROCEEDINGS{reycls98,
	author= {D. A. Reynolds and et. al},
	title = {{B}lind {C}lustering of {S}peech {U}tterances {B}ased on {S}peaker and {L}anguage {C}haracteristics},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3193-3196},
	year={1998}
}

@INPROCEEDINGS{Hermansky98,
	author={S. Van Vuuren and H. Hermansky},
	title={{O}n the {I}mportance of {C}omponents of the {M}odulation {S}pectrum for {S}peaker {V}erification},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3205-3208},
	year = {1998}
}


@Article{Pellom98,
    author={B. L. Pellom and J. H. L. Hansen},
    title={{A}n {E}fficient {S}coring {A}lgorithm for {G}aussian {M}ixture {M}odel {B}ased {S}peaker {I}dentification},
    journal={IEEE Signal Proc. Lett.},
    volume={5},
    pages={281-284},
    year={1998}
}

@Article{HLDA98,
	author= {N. Kumar and A.G. Andreou},
	title={{H}eteroscedastic {D}iscriminant {A}nalysis and {R}educed {R}ank {HMMs} for {I}mproved {S}peech {R}ecognition},
	journal={Speech Communication},
	volume={26},
	pages={283-297},
	year={1998}
}

@INPROCEEDINGS{Isobe99,
	author= {T. Isobe and J. Takahashi},
	title = {{A} {N}ew {C}ohort {N}ormalization using {L}ocal {A}coustic {I}nformation for {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
        pages = {841-844},
	year={1999}
}

@INPROCEEDINGS{McLaugn99,
     author={J. McLaughlin and D. A. Reynolds and T. Gleason},
     title={{A} {S}tudy of {C}omputation {S}peed-ups of the {GMM-UBM} {S}peaker {R}ecognition {S}ystem},
     booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
     pages={1215-1218},
     year={1999}
}

@INPROCEEDINGS{Markowitz99,
	author={J. Markowitz},
       title={{I}eri and {O}ggi {D}omani: {S}peaker {R}ecognition {Y}esterday, {T}oday and tomorrow},
       booktitle = {Proc. of COST250 Workshop on Speacker Recognition in Telephony},
       year={1999}
}


@INPROCEEDINGS{Auckenthaler1999,
author={R. Auckenthaler and  E. Parris and  M. Carey},
title={{I}mproving a {GMM} {S}peaker {V}erification {S}ystem by {P}honetic {W}eighting},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages={313-316},
 year={1999}
}


@Article{kuhn2000,
author="R. Kuhn and J.-C. Junqua and P. Nguyen and N. Niedzielski",
title="{R}apid {S}peaker {A}daptation in {E}igenvoice {S}pace",
journal="IEEE Trans. on Speech and Audio Processing",
volume="8 (6)",
pages="695-707",
year="2000"	
}	  

@Article{reynold00,
  author="D. A. Reynolds and T. F. Quatieri and R. B. Dunn",
  title="{S}peaker Verification using Adapted Gaussian Mixture Models",
  journal="Digital Signal Processing",
  volume="10",
  pages="19-41",
 year="2000"	  
}

@Article{Tnorm00,
 author="R. Auckenthaler and M. Carey and H. Lloyd-Thomas",
 title="{S}core {N}ormalization for {T}ext-{I}ndependent {S}peaker {V}erification {S}ystem",
 journal="Digital Signal Processing",
 Volume="10",
 pages="42-54",
 year="2000"
 }


@INPROCEEDINGS{Wagner00,
     author= {D. Tran and M. Wagner},
     title = {{A} {P}roposed {L}ikelihood {T}ransformation for {S}peaker {V}erification},
     booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
     pages = {1069-1072},
     year={2000}
}


@Article{kishore00,
  author="S. P. Kishore and B. Yegnanarayana",
  title="{S}peaker {V}erification: {M}inimizing the {C}hannel {E}ffects using {A}utoassociative {N}eural {N}etwork {M}odels",
  journal="ICASSP",
  year="2000",
  pages="1101-1104"
}



@INPROCEEDINGS{Heck00,
	author= {R. Teunen and B. Shahshahani and L. Heck},
	title = {{A} {M}odel-based {T}ransformational {A}pproach to {R}obust {S}peaker {R}ecognition},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
        pages = {495-498},
        year={2000}
}

@INPROCEEDINGS{paliwal00,
	author= {B. Wildermoth and K. K. Paliwal},
	title = {{U}se of {V}oicing and {P}itch {I}nformation for {S}peaker {R}ecognition},
	booktitle = {Proc. 8th Australian Intern. Conf. Speech Science and Technology},
	pages = {324-328},
       year={2000}

}


@INPROCEEDINGS{Gadde2000,
	author= {V. R. R. Gadde},
	title = {{M}odeling {W}ord {D}uration},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {601-604},
        year={2000}
}

@INPROCEEDINGS{Wan2000,
	author= {V. Wan and W. M. Campbell},
	title = {{S}upport {V}ector {M}achines for {S}peaker {V}erification and {I}dentification},
	booktitle = {Proc. IEEE Signal Processing Society Workshop Neural Networks},
	pages = {775-784},
	year={2000}
}


@INPROCEEDINGS{Doddington2001,
        author= {G. Doddington},
        title = {{S}peaker {R}ecognition {B}ased on {I}diolectal {D}ifferences {B}etween {S}peakers},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {2521-2524},
        year={2001}
}  


@INPROCEEDINGS{Sturim01,
        author= {D. Sturim and D. A. Reynolds and E. Singer and J. P. Campbell},
        title = {{S}peaker {I}ndexing in {L}arge {A}udio {D}atabases using {A}nchor {M}odels},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {429-432},
        year={2001}
}

@INPROCEEDINGS{Auck01,
       author={R. Auckenthaler and J. S. Masion},
       title={{G}aussian {S}election {a}pplied to {T}ext-{I}ndependent {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={83-88},
       year={2001}
}

@INPROCEEDINGS{Pelecanos01,
       author={J. Pelecanos and S. Sridharan},
       title={{F}eature {W}arping for {R}obust {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={213-218},
       year= {2001}
}


@INPROCEEDINGS{Wang2001,
        author= {J. C. N. Wang and W. H. Tsai and L. S. Lee},
        title = {{E}igen-{MLLR} {C}oefficients as {N}ew {F}eature {P}arameters for {S}peaker {I}dentification},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {1385-1388},
        year={2001}
}


@INPROCEEDINGS{Kajarekar2001,
author= {S. Kajarekar and H. Hermansky},
title = {{S}peaker {V}erification {B}ased on {B}road {P}honetic {C}ategories},
booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
pages={201-206},
year={2001}
}

@INPROCEEDINGS{Glds_ker2002,
	author={W. M. Campbell},
	title={{G}eneralized {L}inear {D}iscriminant {S}equence {K}ernels for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {161-164},
	year={2002}
}


@INPROCEEDINGS{ReynoldsFmap,
	author= {D.A. Reynolds},
	title = {{C}hannel {R}obust {S}peaker {V}erification via {F}eature {M}apping},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {6-10},
        year={2003}
}


@INPROCEEDINGS{Tkinnun03,
    author={T. Kinnunen and E. Karpov and P. Franti},
    title={{A} Speaker Pruning {A}lgorithm for {R}eal-{T}ime {S}peaker {I}dentification},
    booktitle = {Proc. Audio- and Video-Based Biometric Authentication},
    pages={639-646},
        year={2003}
}




@Article{nisteval04,
	author="{T}he {E}valuation {P}lan of NIST 2004 {S}peaker {R}ecognition {C}ampaign.
	http://www.itl.nist.gov/iad/mig//tests/sre/2004/SRE-04\_evalplan{-}v1a.pdf"
}

@INPROCEEDINGS{bonastre04,
        author = {J. F. Bonastre and N. Scheffer and C. Fredouille and D. Matrouf},
        title = {{N}IST'04 {S}peaker {R}ecognition {E}valuation {C}ampaign: {N}ew {LIA} {S}peaker {D}etection {P}lateform based on {ALIZE} {T}oolkit},
        booktitle = {Proc. of NIST 2004 Speaker Recognition Workshop},
        year = {2004},
}

@INPROCEEDINGS{Binma04,
	author = {B. Ma and H. Meng},
	title = {{E}nglish-{C}hinese {b}ilingual {t}ext-independent {s}peaker {v}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Leung04,
	author = {K. Y. Leung and M. W. Mak and S. Y. Kung},
	title = {{A}pplying {a}rticulatory {f}eatures to {t}elephone-based {s}peaker {v}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Kwong04,
	author = {Q.Y. Hong and S. Kwong},
	title = {{D}iscriminative {t}raining for {s}peaker {i}dentification based on {m}aximum {m}odel {d}istance {a}lgorithm},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}


@ARTICLE {Bimbot04,
author = {F. Bimbot and J.-F. Bonastre and others},
journal = {EURASIP Journal on Applied Signal Processing},
pages = {430-451},
title = {A Tutorial on Text-Independent Speaker Verification},
volume = {4},
year = {2004}
}


@INPROCEEDINGS{Louradour05,
	author = {J. Louradour and K. Daoudi and R. Andre-Obrecht},
	title = {{D}iscriminative {P}ower of {T}ransient {F}rames in {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={613-616},
	year={2005}
}



@INPROCEEDINGS{Stolcke05,
	author= {A. Stolcke and L. Ferrer and S. Kajarekar and E. Shriberg and A. Venkataraman},
	title = {{MLLR} {T}ransforms as {F}eatures in {S}peaker {R}ecognition},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {2425-2428},
        year={2005}
}





@Article{kenny05,
author="P. Kenny",
title="{J}oint {F}actor {A}nalysis of {S}peaker and {S}ession {V}ariability : {T}heory and {A}lgorithms",
journal="Technical report CRIM-06/08-13  Montreal, CRIM",
year="2005"
}



@INPROCEEDINGS{AT_norm,
	author= {D. E. Sturim and D.A. Reynolds},
	title = {{S}peaker {A}daptive {C}ohort {S}election for {T}norm in {T}ext-independent {S}peaker {V}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {741-744},
        year={2005}
}	


@INPROCEEDINGS{datadriven05,
	author= {M. Mason and R. Vogt and B. Baker and S. Sridharan},
	title = {{D}ata-{D}riven {C}lustering for {B}lind {F}eature {M}apping in {S}peaker {V}erification},
	booktitle = {Proc. of Interspeech},
         pages = {3109-3112},
        year={2005}
}


@INPROCEEDINGS{ZTnorm05,
	author= {R. Vogt and B. Baker and S. Sridharan},
	title = {{M}odeling {S}ession {V}ariability in {T}ext-{I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {3117-3120},
	year={2005}
}

@INPROCEEDINGS{Adami05,
	author= {André G. Adami},
        title = {{P}rosodic {M}odeling for {S}peaker {R}ecognition based on {S}ub-band {E}nergy {T}emporal {T}rajectories},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {189 - 192},
        year={2005}
}

@INPROCEEDINGS{NAP2005,
	author= {A. Solomonoff and W. M. Campbell and I. Boardman},
	title = {{A}dvances in {C}hannel {C}ompensation for {SVM} {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {629 - 632},
	year={2005}
}
@INPROCEEDINGS{Campbel_GMM_sup06,
author= {W. Campbell and D. Sturim and D. Reynolds and A. Solomonoff},
title = {{SVM} based {S}peaker {V}erification using a {GMM} {S}upervector {K}ernel and {NAP} {V}ariability {C}ompensation},
 booktitle = { Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {97-100},
 year={2006}
}

@INPROCEEDINGS{Goldberger05adistance,
author = {J. Goldberger and H. Aronowitz},
title = {{A} {D}istance {M}easure {B}etween {GMM}s {B}ased on the {U}nscented {T}ransform and its {A}pplication to {S}peaker {R}ecognition},
booktitle = {in Proc. of Interspeech},
pages = {1985-1989},
year = {2005}
}



@INPROCEEDINGS{krause06,
	author = {N. Krause and R. Gazit},
	title ={{SVM}-based {S}peaker {C}lassification in the {GMM} {M}odels {S}pace},
	booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	year ={2006}
}


@INPROCEEDINGS{Noor06,
	  author = { E. Noor and H. Aronowitz},
	  title={{E}fficient {L}anguage {I}dentification using {A}nchor {M}odels and {S}upport {V}ector {M}achines},    
	  booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	  year ={2006}
}



@inproceedings{Schwarz,
author = {Schwarz, P. and Matejka, P. and Cernocky, J.},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages = {325--328},
title = {{H}ierarchical {S}tructures of {N}eural {N}etworks for {P}honeme {R}ecognition},
year = {2006}
}


@INPROCEEDINGS{Binma06,
	author = {B. Ma and D. Zhu and R. Tong and H. Li},
	title={{S}peaker {C}luster {B}ased {GMM} {T}okenization for {S}peaker {R}ecognition},
	booktitle = {Proc. of Interspeech},
        year ={2006},
}


@INPROCEEDINGS{Hazen06,
  author="R. Woo and A. Park and T. J. Hazen",
  title="{T}he {MIT} {M}obile {D}evice {S}peaker {V}erification {C}orpus: {D}ata {C}ollection and {P}reliminary {E}xperiments",
  booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
  pages="1-6",
  year="2006"
}


@Article{Campbell2006,
	author={W. M. Campbell and D. E. Sturim and D. A. Reynolds},
	title={{S}upport {V}ector {M}achines using {GMM} {S}upervectors for {S}peaker {V}erification},
	 journal={IEEE Signal Process. Lett.},
	 volume={13},
	 pages={308-311},
	 year={2006}
}


@Article{Mami06,
	author="Y. Mami and D. Charlet",
	title="{S}peaker {R}ecognition by {L}ocation in the {S}pace of {R}eference {S}peakers",
	journal="Speech Communication",
	volume="48",
	pages="127-141",
	year="2006"
}

@Article{Skosan06,
	author={M. Skosan and D. Mashao},
	title={{M}odified {S}egmental {H}istogram {E}qualization for {R}obust {S}peaker {V}erification},
	journal={Pattern Recogn. Lett.},
        volume={27},
        pages={479–486},
        year={2006}
}	


@INPROCEEDINGS{hatch06,
   author = {A. Hatch and S. Kajarekar and A. Stolcke},
   title={{W}ithin-{C}lass {C}ovariance {N}ormalization for {SVM}-{B}ased {S}peaker {R}ecognition},
   booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
   pages = {1471-1474},
   year ={2006}
}


@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} {B}ook",
  journal={Copyright 2001-2006 Cambridge University Engineering Department}
   }


@Article{Castro2007,
      author="D. R. Castro and et. al",
      title="{S}peaker {V}erification using {S}peaker- and {T}est-dependent {F}ast {S}core {N}ormalization",
      journal="Pattern Recogn. Lett.",
      volume="28",
      pages="90-98",
      year="2007"
}

@INPROCEEDINGS{Charbuillet07,
	author={C. Charbuillet and B. Gas and M. Chetouani and J. L. Zarader},
	title={{C}omplementary {F}eatures for {S}peaker {V}erification based on {G}enetic {A}lgorithms},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={285-288},
	year = {2007}
}

@INPROCEEDINGS{Xugang07,
	author={X. Lu and J. Dang},
	 title={{P}hysiological {F}eature {E}xtraction for {T}ext {I}ndependent {S}peaker {I}dentification using {N}on-{U}niform {S}ub-band {P}rocessing},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={461-464},
        year = {2007}
}

@INPROCEEDINGS{Saeidi07,
	author={R. Saeidi and H. R. Sadegh Mohammadi and R. D. Rodman and T Kinnunen},
	title={{A} {N}ew {S}egmentation {A}lgorithm {C}ombined with {T}ransient {F}rames {P}ower for {T}ext {I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={305-308},
	year = {2007}
}
		
@INPROCEEDINGS{Tur2007,
	author={G. Tur and E. Shriberg and A. Stolcke and S. Kajarekar},
	title={{D}uration and {P}ronunciation {C}onditioned {L}exical {M}odeling for {S}peaker {S}erification},
        booktitle = {Proc. of Interspeech},
	pages={2049-2052},
	year = {2007}
}

@Article{HLDA_feat07,
	author={L. Burget and  P. Matejka and  O. Glembek and P. Schwarz and J. Cernocky},
        title = {{A}nalysis of {F}eature {E}xtraction and {C}hannel {C}ompensation in {GMM} {S}peaker {R}ecognition {S}ystem},
	journal={IEEE Trans. on Audio, Speech, Lang. Process.},
	volume={15},
	pages={1979-1986},
	year={2007}
}

@Article{fusion_2007,
	 author={N. Brummer and L. Burget and J. Cernocky and others},
	 title = {{F}usion of {H}eterogeneou {S}peaker {R}ecognition {S}ystems in the {STBU} {S}ubmission for the {NIST} {S}peaker {R}ecognition {E}valuation 2006},
	 journal={IEEE Trans. on Audio, Speech, and Lang. Process.},
	 volume={15},
	 pages={2072-2084},
	 year={2007}
}

@INPROCEEDINGS{Hazen97,
       author= {T. J. Hazen and J. R. Glass},
       title = {{A} {C}omparison of {N}ovel {T}echniques for {I}nstantaneous {S}peaker {A}daptation},
       booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
       pages = {2047-2050},
       year = {1997}
}


@INPROCEEDINGS{ferras-icassp08,
	author = {M. Ferras and  C. C. Leung and C. Barras and J. L. Gauvain},
        title = {{C}onstrained {MLLR} for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {53-56},
	year = {2007}
}


	       


@inproceedings{akhil-interspeech2008,
      author = {P. T. Akhil and S. P. Rath and S. Umesh and D. R. Sanand},
      title = {{A} {C}omputationally {E}fficient {A}pproach to {W}arp {F}actor {E}stimation in {VTLN} Using {EM} {A}lgorithm and {S}ufficient {S}tatistics},
      booktitle = {Proc. of Interspeech},
      pages = {1713-1716},
      year = {2008}
}


@inproceedings{sanand-interspeech2008,
      author={D. R. Sanand and S. Umesh},
      title={{S}tudy of {J}acobian {C}ompensation Using {L}inear {T}ransformation of {C}onventional {MFCC} for {VTLN}},
      booktitle={Proc. of Interspeech},
      pages={1233-1236},
      year={2008}
}




@inproceedings{Yossi09,
	author = {Y. Bar-Yosef and Y. Bistritz},
        title = {{A}daptive {I}ndividual {B}ackground {M}odel for {S}peaker {V}erification},
        booktitle = {Proc. of Interspeech},
	pages = {1271-1274},
	year = {2009}
}	

@Article{Vraj09,
	author="V. R. Apsingekar and P. L. De Leon",
	title="{S}peaker {M}odel {C}lustering for {E}fficient {S}peaker {I}dentification in {L}arge {P}opulation {A}pplications",
	journal="IEEE Trans. on Speech and Language Processing",
	volume="17",
	pages="848-853",
	year="2009"
}


@article{kinnunen2010overview,
  title={{A}n Overview Of Text-independent Speaker Recognition: From Features To Supervectors},
  author={Kinnunen, T. and Li, H.},
  journal={Speech communication},
  volume={52},
  number={1},
  pages={12--40},
  year={2010}
 }



@inproceedings{achintya-odyssey2010,
	author= {A. K. Sarkar and S. Umesh},
	title= {{I}nvestigation of {S}peaker-{C}lustered {UBM}s based on {V}ocal {T}ract {L}engths and {MLLR} matrices for {S}peaker {V}erification},
	booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	pages= {286-293},
	year = {2010}

}

@inproceedings{achintya-odyssey2010_spkid,
	      author= {A. K. Sarkar and S. Umesh and S. P. Rath},
	      title= {{C}omputationally {E}fficient {S}peaker {I}dentification for {L}arge {P}opulation {T}asks using {MLLR} and {S}ufficient {S}tatistics},
	      booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	      pages= {7-11},
              year = {2010}
}


@inproceedings{Zhang-odyssey2010,
       author= {W. Q. Zhang and Y. Shan and J. Liu},
       title= {{M}ultiple {B}ackground {M}odels for {S}peaker {V}erification},
       booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={47-51},
       year = {2010}
}


@inproceedings{achintya-inter2010,
             author= {A. K. Sarkar and S. Umesh},
             title= {{F}ast {C}omputation of {S}peaker {C}haracterization {V}ector using {MLLR} and {S}ufficient {S}tatistics in {A}nchor {M}odel {F}ramework},
             booktitle = {Proc. of Interspeech},
	     pages={2738-2741},
	     year = {2010}
}


@inproceedings{achintya-icassp2011,
	        author= {A. K. Sarkar and S. Umesh},
	        title= {{U}se of {VTL}-wise {M}odels in {F}eature-{M}apping {F}ramework to {A}chieve {P}erformance of {M}ultiple-{B}ackground {M}odels in {S}peaker {V}erification},
	        booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
		pages={4552-4555},
	        year = {2011}

}

@inproceedings{SenoussaouiInterspch2011,
        author= {M. Senoussaoui and others},
        title= {{M}ixture of {PLDA} {M}odels {I}n {I}-{V}ector {S}pace {F}or {G}ender-{I}ndependent {S}peaker {R}ecognition},
        booktitle={Proc. of Interspeech},
        pages={25-28},
         year = {2011}
}


@Article{Deka_ieee2011,
       author= {N. Dehak and P. Kenny and R. Dehak and P. Ouellet and P. Dumouchel},
       title= {{F}ront-End Factor Analysis for Speaker Verification},
       journal={IEEE Trans. on Audio, Speech and Language Processing},
       volume={19},
       pages={788-798},
       year = {2011}
}

@inproceedings{Romero2011,
        author= {D. G. Romero and C. Y. Espy-Wilson},
        title= {{A}nalysis of i-vector {L}ength {N}ormalization in {S}peaker {R}ecognition {S}ystems},
        booktitle={Proc. of Interspeech},
        pages={249-252},
        year={2011}
}



@inproceedings{Kanagasundaram2011,
author={A. Kanagasundaram and R. Vogt and D. Dean and  S. Sridharan and M. Mason},
title= {i-vector based {S}peaker {R}ecognition on {S}hort {U}tterances},
booktitle={Proc. of Interspeech},
pages={2341-2344},
year={2011}
}

@inproceedings{Pierre-interspeech2012,
       author= {P. M. Bousquet and others},
       title= {{V}ariance-{S}pectra {B}ased {N}ormalization {F}or i-vector {S}tandard {A}nd {P}robabilistic {L}inear {D}iscriminant {A}nal
ysis},
       booktitle={Proc. of  Odyssey Speaker and Language Recognition Workshop},
       year={2012}
}

@inproceedings{Larcher2012,
author= {A. Larcher and K. A. Lee and  B. Ma and H. Li},
title= {{RSR2015}: {D}atabase for {T}ext-dependent {S}peaker {V}erification using {M}ultiple {P}ass-phrases},
booktitle={Proc. of Interspeech},
pages={1580-1583},
 year = {2012}
}

@inproceedings{achintya2012,
author={A. K. Sarkar and  D. Matrouf and P. M. Bousquet and J. F. Bonastre},
title= {{S}tudy of the Effect of i-vector Modeling on Short and Mismatch Utterance Duration for Speaker Verification},
booktitle={Proc. of Interspeech},
pages={2662-2665},
year={2012}
}




@inproceedings{Plchot2013,
author={O. Plchot and others},
title={{D}eveloping  a  {S}peaker  {I}dentification {S}ystem  for the {DARPA} {RATS} {P}roject},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages={ 6768-6772},
year={2013}
}





@inproceedings{Fu2014,
author={T. Fu and Y. Qian and Y. Liu and Kai Yu}, 
title= {{T}andem {D}eep {F}eatures for {T}ext-dependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1327-1331},
year = {2014}
}

@inproceedings{Nicolas2014,
author={N. Scheffer and Y. Lei},
title= {{C}ontent {M}atching for {S}hort {D}uration {S}peaker {R}ecognition},
booktitle={Proc. of Interspeech},
pages={1317-1321},
year = {2014}
}

@inproceedings{Hagai2014,
author={H. Aronowitz and  A. Rendel},
title= {{D}omain {A}daptation for {T}ext {D}ependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1337-1341},
year = {2014}
}


@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent {S}peaker {V}erification: {C}lassifiers, {D}atabases and {RSR2015}},
journal={Speech Communucation},
volume={60},
pages={56-77},
year={2014}
}


@inproceedings{McLaren2015,
author={M. McLaren and Y. Lei and L. Ferrer},
title={{A}dvances {I}n {D}eep {N}eural {N}etwork {A}pproaches {T}o {S}peaker {R}ecognition},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2015}
}


@Article{Yuan2015,
author={Y. Liu and Y. Qian and N. Chen and T. Fu and Y. Zhang and K. Yu},
title= {{D}eep {F}eature for {T}ext-dependent {S}peaker {V}erification},
journal={Speech Communication},
volume={73},
pages={1-13},
year={2015}
}

@inproceedings{Delgado2016Asru,
author={H. Delgado and  M. Todisco and  M. Sahidullah and  A. K. Sarkar and N. Evans and  T. Kinnunen and  Z.-H. Tan},
title={{F}URTHER OPTIMISATIONS OF CONSTANT Q CEPSTRAL PROCESSING FOR INTEGRATED UTTERANCE AND TEXT-DEPENDENT SPEAKER VERIFICATION},
booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)},
year={2016}
}

@misc{CNTK,
author= {A. Agarwal and others},
title= {{A}n {I}ntroduction to {C}omputational {N}etworks and the {C}omputational {N}etwork {T}oolkit},
year={2016},
howpublished ={https://www.microsoft.com/en-us/research/publication/an-introduction-to-computational-networks-and-the-computational-network-toolkit/}
}

@article{Tang2016,
author = {H. Tang},
title= {{S}equence {P}rediction with {N}eural {S}egmental {M}odels},
journal = {Ph.D. dissertation, Dept. Comput. Sci., Toyota Technological Inst. Chicago,
Chicago, IL, USA},
year =  {2017}
}


@inproceedings{yu2017adversarial,
  title={{A}dversarial {N}etwork {B}ottleneck {F}eatures {F}or {N}oise {R}obust {S}peaker {V}erification},
  author={Yu, H. and Tan, Z.-H. and Ma, Z. and Guo, J.},
  booktitle={Proc. of Interspeech},
  pages={1492--1496},
  year={2017}
}



@article{tang2017endtoend,
  title = {{E}nd-to-End {N}eural {S}egmental {M}odels {F}or {S}peech {R}ecognition},
  author = {H. Tang and L. Lu and K. Gimpel and K. Livescu and C. Dyer and N. A. Smith and S. Renals},
  year = {2017},
  pages={1254-1264},
  journal = {IEEE Journal of Selected Topics in Signal Processing},
  volume = {11}
}



@article{DBLP:journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and
               Z.-H. Tan and
               H. Tang and
               S. Shon and
               J. R. Glass},
  title     = {{T}ime-Contrastive Learning Based Deep Bottleneck Features for Text-Dependent Speaker Verification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}

@misc{xvector_recipe,
 title= {https://github.com/kaldi-asr/kaldi/tree/master/egs/sre16/v2}
 }
 
@inproceedings{conf/icassp/SnyderGSPK18,
  author    = {D. Snyder and
               D. Garcia{-}Romero and
               G. Sell and
               D. Povey and
               S. Khudanpur},
  title     = {{X}-Vectors: Robust DNN Embeddings for Speaker Recognition},
  booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages     = {5329--5333},
   year      = {2018}
}


@Article{alizetoolkit,
  title="http://lia.univ-avignon.fr/heberges/ALIZE/"
   }

@Article{mit_database,
  title="http://groups.csail.mit.edu/sls/mdsvc"
}

@Book{duda_hart_patt,
	  author = {R.O. Duda and P.E. Hart and D.G. Stork},
	  title  = {{P}attern {C}lassification},
	  publisher = {New York: John Wiley \& Sons},
	  year    = {2001}
}


@inproceedings{Timit,
author = {J. S. Garofolo and L. F. Lamel and W. M. Fisher and J. G. Fiscus and  D. S. Pallett and N. L. Dahlgren and V. Zue},
title = {{TIMIT} {A}coustic-{P}honetic {C}ontinuous {S}peech {C}orpus {LDC}93{S}1},
publisher = {Web Download. Philadelphia: Linguistic Data Consortium},
year={1993}
}


@inproceedings{noise_mix,
author= {A. Hannun and C. Case and J. Casper and B. Catanzaro and G. Diamos and E. Elsen and R. Prenger and S. Satheesh and S. Sengupta and A. Coates and A. Ng},
title = {{D}eep Speech: Scaling Up End-to-End Speech recognition},
 booktitle= {in arXiv, 2014}
}


@article{Sarkar2017,
author = {A. K. Sarkar and Z.-H. Tan},
title ={{I}ncorporating {P}ass-phrase {D}ependent {B}ackground {M}odels for {T}ext-dependent {S}peaker {V}erification},
journal={ Computer speech \& Language},
volume={47},
year ={2018},
pages= {259-271}
}



@article{journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and Z. -H. Tan and H. Tang and S. Shon and  J. R. Glass},
  title     = {{T}ime-Contrastive Learning Based Deep Bottleneck Features for Text-Dependent Speaker Verification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}


@article{TanSD20,
  author    = {Z.-H. Tan and  A. K. Sarkar and N. Dehak},
  title     = {{rVAD}: An Unsupervised Segment-based Robust Voice Activity Detection Method},
  journal   = {Computer Speech \& Language},
  volume    = {59},
  pages     = {1--21},
  year      = {2020}

 } 



@article{Park_2019,
   title={{S}pecAugment: A Simple Data Augmentation Method for Automatic Speech Recognition},
    pages={2613--2617},
   author={Park, D. S. and Chan, W. and Zhang, Y. and Chiu, C.-C. and Zoph, B. and Cubuk, E. D. and Le, Q. V.},
   year={2019},
   booktitle={Proc. of Interspeech}
}

@INPROCEEDINGS{Jaitly_vocaltract,
    author = {N. Jaitly and G. E. Hinton},
    title = {{V}ocal Tract Length Perturbation (VTLP) Improves Speech Recognition},
    booktitle = {In International Conference on Machine Learning (ICML)},
    year = {2013}
}

@INPROCEEDINGS{Mauch2013,
author = {M. Mauch and S. Ewert},
title = {{T}he Audio Degradation Toolbox and its Application to Robustness Evaluation},
year = {2013},
booktitle = {International Society for Music Information Retrieval Conference, ISMIR},
pages = {83-88}
}

@INPROCEEDINGS{Lasseck2018,
author = {M. Lasseck},
title= {{A}udio-based Bird Species Identification with Deep Convolutional Neural Networks},
booktitle = {In: Working Notes of CLEF 2018 (C{r}oss Lan{g}uage Evaluation Fo{r}um)}
}


@misc{Focal,
	author= {N. Brummer},
	title= {{F}oCal {T}oolkit},
       howpublished ={Available at http://sites.google.com/site/nikobrummer/focal}
}

@misc{Lnknet,
title= {http://www.ll.mit.edu/mission/communications/ist/lnknet/index.html}
}
@misc{RedDots,
title= {The RedDots Challenge: Towards Characterizing Speakers from Short Utterances},
howpublished ={https://sites.google.com/site/thereddotsproject/reddots-challenge}
}

@misc{SRE08,
title = {https://www.nist.gov/itl/iad/mig/2008-nist-speaker-recognition-evaluation-results}
}

@ARTICLE{7829341,
author={J. {Salamon} and J. P. {Bello}},
journal={IEEE Signal Processing Letters},
title={{D}eep Convolutional Neural Networks and Data Augmentation for Environmental Sound Classification},
year={2017},
volume={24}, 
number={3},
pages={279-283}
}


@ARTICLE{24792,  
author={F. L. {Bookstein}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},  
title={{P}rincipal Warps: Thin-plate Splines and the Decomposition of Deformations},
year={1989}, 
volume={11},
number={6}, 
pages={567-585}
}

@ARTICLE{Shorten2019,
author = {C. Shorten and T. M. Khoshgoftaar},
title = {{A} Survey on Image Data Augmentation for Deep Learning},
journal = {Journal of Big Data},
year ={2019}
}


@INPROCEEDINGS{ITU2005,
author = {ITU},
title = {{G.} 191: Software Tools for Speech and Audio Coding Standardization},
booketitle ={International Telecommunication Union},
year = {2005}

}



@INPROCEEDINGS{7528399,  
author={H. {Yu} and A. {Sarkar} and D. A. L. {Thomsen} and Z. {Tan} and Z. {Ma} and J. {Guo}},
booktitle={First International Workshop on Sensing, Processing and Learning for Intelligent Machines (SPLINE)},  
title={{E}ffect of Multi-condition Training and Speech Enhancement Methods on Spoofing Detection},
year={2016}, 
pages={1-5}
}

@INPROCEEDINGS{I4U2013,
author = {R. Saeidi and others},
title = {{I4U} Ssubmission to NIST SRE 2012: A Large-scale Collaborative Effort for Noise-robust Speaker Verification},
pages= {1986-1990},
year ={2013},
Booktitle = {Proc. of Interspeech}
}

@INPROCEEDINGS{Stewart2010,
author = {R. Stewart and M. Sandler},
title = {{D}atabase of Omnidirectional and b-format Room Impulse Responses},
booktitle = {In Proc. IEEE Intl. Conf. on Acoustics Speech and Signal Processing (ICASSP)},
pages = {165-168},
year={2010}
}

@inproceedings{Hinton2012,
author = {G. Hinton and others},
title = {{D}eep {N}eural {N}etworks {F}or {A}coustic {M}odeling {I}n {S}peech {R}ecognition},
booktitle={IEEE Signal Process. Mag.},
pages={82-97},
year={2012}
}

